Differentiable Feature Selection, a Reparameterization Approach

We consider the task of feature selection for reconstruction which consists in choosing a small subset of features from which whole data instances can be reconstructed. This is of particular importance in several contexts involving for example costly physical measurements, sensor placement or information compression. To break the intrinsic combinatorial nature of this problem, we formulate the task as optimizing a binary mask distribution enabling an accurate reconstruction. We then face two main challenges. One concerns differentiability issues due to the binary distribution. The second one corresponds to the elimination of redundant information by selecting variables in a correlated fashion which requires modeling the covariance of the binary distribution. We address both issues by introducing a relaxation of the problem via a novel reparameterization of the logitNormal distribution. We demonstrate that the proposed method provides an effective exploration scheme and leads to efficient feature selection for reconstruction through evaluation on several high dimensional image benchmarks. We show that the method leverages the intrinsic geometry of the data, facilitating reconstruction.

==> source/arxive.tex <==
\section{about the other way round}
\subsubsection{Optimization Procedure}
To perform the optimization of \cref{eq.min_l2}, we rely on the basic differential multiplier method \cite{Platt1987}.
This method have theoretically convergence guarantees for example in quadratic optimization.
Unlike, Uzawa's multiplier method, requiring an increasing sequence of Lagrange multiplier diverging to $+\infty$, this method simply ascend the gradient with relation to this multiplier, gradually forcing $G$ and $s$ to satisfy the reconstruction constraint.

Let $\lambda>0$, the desired level of reconstruction desired. We first need to build the Lagrangian problem of \cref{eq.min_l2}:
\begin{equation}
    \mathcal{L}_{\ell_2}(\mu) = ||s||_0 - \mu (\lambda - ||G(s\odot x) - x||_2)
\end{equation}

\begin{algorithm}
\SetAlgoLined
\hspace*{\algorithmicindent} \textbf{Input:} $\lambda, \eta_\theta, \eta_\mu, \eta_\mu>0$,  \\
\hspace*{\algorithmicindent} \textbf{Output:}Converged $s_\theta$ and $G_\psi$\\
 \hspace*{\algorithmicindent} \textbf{Initialization:} $s_\theta$ and $G_\psi$, and set $\mu=10^{-8}$ \\
 \While{Convergence not reached}{
    Update $s_\theta$, $G_\psi$ and $\mu$ according to:
    \begin{equation*}
    \begin{aligned}
        &\theta^{k+1} = \theta^{k} - \eta_\theta \frac{\partial \mathcal{L}_{\ell_2}(\mu^k)}{\partial \theta} \\
        &\psi^{k+1} = \psi^{k} - \eta_\psi \frac{\partial \mathcal{L}_{\ell_2}(\mu^k)}{\partial \psi} \\
        &\mu^{k+1} = \mu^{k} + \eta_\mu \frac{\partial \mathcal{L}_{\ell_2}(\mu^k)}{\partial \mu}
    \end{aligned}
    \end{equation*}
  $k\leftarrow k + 1$ \;
  }
 \caption{Reconstruction Controlled Sparsity}
  \label{algo.general}
\end{algorithm}


Let $(s_\theta, G_\psi)$ be a parameterization of $(s, G)$ respectively the sampling operator and the reconstruction operator. The optimization procedure, relying on gradient descend on  $(s_\theta, G_\psi)$ and gradient ascent on $\mu$ can be summarized by \cref{algo.general}.


\paragraph{Interpretation}
Conventionally, other approaches increase the penalty on the sparse term of the loss function to increase sparsity \cref{l0, ...}, instead our proposition, summarized in \cref{algo.general}, indicates that we aim at controlling the level of desired reconstruction. 
Moreover, any level of reconstruction can be reached: from $\lambda=0$ which will consists in observing all pixels to the peak, to no observations at all, making $G$ output the pixel average.

\begin{enumerate}
    \item Does the distribution collapse ==> to a fixed mask ?
    \item Fixed thresholding ?
\end{enumerate}


\paragraph{Learning the dynamics:}
it learns first how to generates sparse masks, then which point to make emerge.
maybe schedule the weight.

